A deeper look at depth pruning of LLMs

Large Language Models (LLMs) are not only resource-intensive to train but even more costly to deploy in production. Therefore, recent work has attempted to prune blocks of LLMs based on cheap proxies for estimating block importance, effectively removing 10% of blocks in well-trained LLaMa-2 and Mistral 7b models without any significant degradation of downstream metrics. In this paper, we explore different block importance metrics by considering adaptive metrics such as Shapley value in addition to static ones explored in prior work. We show that adaptive metrics exhibit a trade-off in performance between tasks i.e., improvement on one task may degrade performance on the other due to differences in the computed block influences. Furthermore, we extend this analysis from a complete block to individual self-attention and feed-forward layers, highlighting the propensity of the self-attention layers to be more amendable to pruning, even allowing removal of upto 33% of the self-attention layers without incurring any performance degradation on MMLU for Mistral 7b (significant reduction in costly maintenance of KV-cache). Finally, we look at simple performance recovery techniques to emulate the pruned layers by training lightweight additive bias or low-rank linear adapters. Performance recovery using emulated updates avoids performance degradation for the initial blocks (up to 5% absolute improvement on MMLU), which is either competitive or superior to the learning-based technique.

==> figures/adapter_loss/training_loss_llama2_rank_256.tex <==
\begin{figure}[t]
    \centering
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_0.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_1.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_2.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_3.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_4.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_5.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_6.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_7.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_8.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_9.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_10.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_11.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_12.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_13.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_14.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_15.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_16.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_17.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_18.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_19.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_20.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_21.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_22.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_23.pdf}
    }

    \caption{\textbf{Low-rank linear adapter training curves for the first 24 LLaMa-2 7b blocks with a rank of 256} trained using three different objectives including (a) MSE loss defined on the representation, (b) supervised fine-tuning (SFT), and (c) logit distillation where logits are distilled from the full model. Rest of the blocks are visualized in Fig.~\ref{fig:linear_adapters_rank_256_llama2_train_loss_b}.}
    \label{fig:linear_adapters_rank_256_llama2_train_loss_a}
\end{figure}


\begin{figure}[t]
    \centering
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_24.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_25.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_26.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_27.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_28.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_29.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_30.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_256/loss_llama-2_rank_256_block_idx_31.pdf}
    }

    \caption{\textbf{Low-rank linear adapter training curves for the last 8 LLaMa-2 7b blocks with a rank of 256} trained using three different objectives including (a) MSE loss defined on the representation, (b) supervised fine-tuning (SFT), and (c) logit distillation where logits are distilled from the full model. The first set of blocks are visualized in Fig.~\ref{fig:linear_adapters_rank_256_llama2_train_loss_a}.}
    \label{fig:linear_adapters_rank_256_llama2_train_loss_b}
\end{figure}


==> figures/adapter_loss/training_loss_llama2_rank_32.tex <==
\begin{figure}[t]
    \centering
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_0.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_1.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_2.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_3.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_4.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_5.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_6.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_7.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_8.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_9.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_10.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_11.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_12.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_13.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_14.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_15.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_16.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_17.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_18.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_19.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_20.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_21.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_22.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_23.pdf}
    }

    \caption{\textbf{Low-rank linear adapter training curves for the first 24 LLaMa-2 7b blocks with a rank of 32} trained using three different objectives including (a) MSE loss defined on the representation, (b) supervised fine-tuning (SFT), and (c) logit distillation where logits are distilled from the full model. Rest of the blocks are visualized in Fig.~\ref{fig:linear_adapters_rank_32_llama2_train_loss_b}.}
    \label{fig:linear_adapters_rank_32_llama2_train_loss_a}
\end{figure}


\begin{figure}[t]
    \centering
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_24.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_25.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_26.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_27.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_28.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_29.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_30.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_32/loss_llama-2_rank_32_block_idx_31.pdf}
    }

    \caption{\textbf{Low-rank linear adapter training curves for the last 8 LLaMa-2 7b blocks with a rank of 32} trained using three different objectives including (a) MSE loss defined on the representation, (b) supervised fine-tuning (SFT), and (c) logit distillation where logits are distilled from the full model. The first set of blocks are visualized in Fig.~\ref{fig:linear_adapters_rank_32_llama2_train_loss_a}.}
    \label{fig:linear_adapters_rank_32_llama2_train_loss_b}
\end{figure}


==> figures/adapter_loss/training_loss_llama2_rank_8.tex <==
\begin{figure}[t]
    \centering
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_0.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_1.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_2.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_3.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_4.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_5.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_6.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_7.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_8.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_9.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_10.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_11.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_12.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_13.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_14.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_15.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_16.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_17.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_18.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_19.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_20.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_21.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_22.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_23.pdf}
    }

    \caption{\textbf{Low-rank linear adapter training curves for the first 24 LLaMa-2 7b blocks with a rank of 8} trained using three different objectives including (a) MSE loss defined on the representation, (b) supervised fine-tuning (SFT), and (c) logit distillation where logits are distilled from the full model. Rest of the blocks are visualized in Fig.~\ref{fig:linear_adapters_rank_8_llama2_train_loss_b}.}
    \label{fig:linear_adapters_rank_8_llama2_train_loss_a}
\end{figure}


\begin{figure}[t]
    \centering
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_24.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_25.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_26.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_27.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_28.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_29.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_30.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/llama-2_rank_8/loss_llama-2_rank_8_block_idx_31.pdf}
    }

    \caption{\textbf{Low-rank linear adapter training loss curves for the last 8 LLaMa-2 7b blocks with a rank of 8} trained using three different objectives including (a) MSE loss defined on the representation, (b) supervised fine-tuning (SFT), and (c) logit distillation where logits are distilled from the full model. The first set of blocks are visualized in Fig.~\ref{fig:linear_adapters_rank_8_llama2_train_loss_a}.}
    \label{fig:linear_adapters_rank_8_llama2_train_loss_b}
\end{figure}


==> figures/adapter_loss/training_loss_mistral_rank_256.tex <==
\begin{figure}[t]
    \centering
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_0.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_1.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_2.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_3.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_4.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_5.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_6.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_7.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_8.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_9.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_10.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_11.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_12.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_13.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_14.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_15.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_16.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_17.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_18.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_19.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_20.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_21.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_22.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_23.pdf}
    }

    \caption{\textbf{Low-rank linear adapter training curves for the first 24 Mistral 7b blocks with a rank of 256} trained using three different objectives including (a) MSE loss defined on the representation, (b) supervised fine-tuning (SFT), and (c) logit distillation where logits are distilled from the full model. Rest of the blocks are visualized in Fig.~\ref{fig:linear_adapters_rank_256_llama2_train_loss_b}.}
    \label{fig:linear_adapters_rank_256_mistral_train_loss_a}
\end{figure}


\begin{figure}[t]
    \centering
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_24.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_25.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_26.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_27.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_28.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_29.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_30.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_256/loss_mistral_rank_256_block_idx_31.pdf}
    }

    \caption{\textbf{Low-rank linear adapter training curves for the last 8 Mistral 7b blocks with a rank of 256} trained using three different objectives including (a) MSE loss defined on the representation, (b) supervised fine-tuning (SFT), and (c) logit distillation where logits are distilled from the full model. The first set of blocks are visualized in Fig.~\ref{fig:linear_adapters_rank_256_llama2_train_loss_a}.}
    \label{fig:linear_adapters_rank_256_mistral_train_loss_b}
\end{figure}


==> figures/adapter_loss/training_loss_mistral_rank_32.tex <==
\begin{figure}[t]
    \centering
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_0.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_1.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_2.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_3.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_4.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_5.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_6.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_7.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_8.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_9.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_10.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_11.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_12.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_13.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_14.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_15.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_16.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_17.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_18.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_19.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_20.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_21.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_22.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_23.pdf}
    }

    \caption{\textbf{Low-rank linear adapter training curves for the first 24 Mistral 7b blocks with a rank of 32} trained using three different objectives including (a) MSE loss defined on the representation, (b) supervised fine-tuning (SFT), and (c) logit distillation where logits are distilled from the full model. Rest of the blocks are visualized in Fig.~\ref{fig:linear_adapters_rank_32_llama2_train_loss_b}.}
    \label{fig:linear_adapters_rank_32_mistral_train_loss_a}
\end{figure}


\begin{figure}[t]
    \centering
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_24.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_25.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_26.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_27.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_28.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_29.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_30.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_32/loss_mistral_rank_32_block_idx_31.pdf}
    }

    \caption{\textbf{Low-rank linear adapter training curves for the last 8 Mistral 7b blocks with a rank of 32} trained using three different objectives including (a) MSE loss defined on the representation, (b) supervised fine-tuning (SFT), and (c) logit distillation where logits are distilled from the full model. The first set of blocks are visualized in Fig.~\ref{fig:linear_adapters_rank_32_llama2_train_loss_a}.}
    \label{fig:linear_adapters_rank_32_mistral_train_loss_b}
\end{figure}


==> figures/adapter_loss/training_loss_mistral_rank_8.tex <==
\begin{figure}[t]
    \centering
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_0.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_1.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_2.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_3.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_4.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_5.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_6.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_7.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_8.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_9.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_10.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_11.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_12.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_13.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_14.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_15.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_16.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_17.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_18.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_19.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_20.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_21.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_22.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_23.pdf}
    }

    \caption{\textbf{Low-rank linear adapter training curves for the first 24 Mistral 7b blocks with a rank of 8} trained using three different objectives including (a) MSE loss defined on the representation, (b) supervised fine-tuning (SFT), and (c) logit distillation where logits are distilled from the full model. Rest of the blocks are visualized in Fig.~\ref{fig:linear_adapters_rank_8_llama2_train_loss_b}.}
    \label{fig:linear_adapters_rank_8_mistral_train_loss_a}
\end{figure}


\begin{figure}[t]
    \centering
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_24.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_25.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_26.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_27.pdf}
    }


    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_28.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_29.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_30.pdf}
    }
    \subfloat{
        \includegraphics[width=0.245\textwidth]{figures/adapter_loss/mistral_rank_8/loss_mistral_rank_8_block_idx_31.pdf}
    }

    \caption{\textbf{Low-rank linear adapter training curves for the last 8 Mistral 7b blocks with a rank of 8} trained using three different objectives including (a) MSE loss defined on the representation, (b) supervised fine-tuning (SFT), and (c) logit distillation where logits are distilled from the full model. The first set of blocks are visualized in Fig.~\ref{fig:linear_adapters_rank_8_llama2_train_loss_a}.}
    \label{fig:linear_adapters_rank_8_mistral_train_loss_b}
\end{figure}


==> sections/abstract.tex <==
\begin{abstract}
% Large Language Models (LLMs) are not only resource-intensive to train but even more costly to deploy in production.
% Therefore, recent work has attempted to prune blocks of LLMs based on cheap proxies for estimating block importance, effectively removing 10\% blocks of well-trained LLaMa-2 and Mistral models with just 7b parameters.
% In this paper, we attempt to better understand the utility of different block importance metrics by considering dynamic metrics such as Shapley value in addition to static ones explored in prior work.
% Contrary to prior work, we show that dynamic metrics highlight a trade-off in performance between tasks due to differences in block influences.
% Furthermore, we extend this analysis from full blocks to individual self-attention and feed-forward layers, and highlight the propensity of the self-attention layers to be more amendable to pruning, even allowing removal of upto 40\% of the self-attention layers without incurring any performance degradation for Mistral 7b (significant reduction in costly maintenance of KV-cache).
% Finally, we look at simple performance recovery techniques such as a simple additive bias (emulated update) as well as training of linear adapters.
% Our analysis shows that simple techniques such as emulated updates provide significant gains in avoiding performance degradation (upto 5\% on MMLU) that are comparable to learning-based techniques.
% However, none of the explored techniques are effectively able to delay the severe performance degradation, highlighting a strong boundary between relevant and irrelevant blocks.

Large Language Models (LLMs) are not only resource-intensive to train but even more costly to deploy in production.
Therefore, recent work has attempted to prune blocks of LLMs based on cheap proxies for estimating block importance, effectively removing 10\% of blocks in well-trained LLaMa-2 and Mistral 7b models without any significant degradation of downstream metrics.
In this paper, we explore different block importance metrics by considering adaptive metrics such as Shapley value in addition to static ones explored in prior work.
We show that \textit{adaptive metrics exhibit a trade-off in performance between tasks i.e., improvement on one task may degrade performance on the other due to differences in the computed block influences}.
Furthermore, we extend this analysis from a complete block to individual self-attention and feed-forward layers, highlighting the propensity of the self-attention layers to be more amenable to pruning, even allowing \textit{\textbf{removal of up to 33\% of the self-attention layers without incurring any performance degradation on MMLU for Mistral 7b}} (significant reduction in costly maintenance of KV-cache).
Finally, we look at simple performance recovery techniques to emulate the pruned layers by training lightweight additive bias or low-rank linear adapters.
% that can be trained efficiently even on a single GPU.
\textit{Performance recovery using emulated updates avoids performance degradation for the initial blocks (up to 5\% absolute improvement on MMLU)}, which is either competitive or superior to the learning-based technique.
\end{abstract}

% Keywords: LLMs, depth pruning, block influence estimation

% TL;DR: This paper investigates different metrics that can be used to identify block importance that is subsequently used to prune irrelevant ones from an LLM.

==> sections/broader_impact.tex <==
\section{Broader Impact}

This work attempts to analyze the contribution of different blocks of a network, which can in turn enable more efficient inference by removing irrelevant blocks at inference time.
Democratizing access to these powerful systems can ensure equal advantage to different groups, including ones with limited computation resources.
On the other hand, making these models more efficient for consumer hardware carries the same risk of intentional bad use such as cyberwarfare, persuasion, and production of fake information.
However, these risks are not unique to our work, but rather, shared with all attempts to make these models more accessible to a broader audience.


==> sections/conclusion.tex <==
\section{Conclusion}

% This paper explores the depth pruning of LLMs.
% We explore and highlight the difference in performance with different influence techniques, including adaptive ones in contrast to prior work.
% We show that block-sensitivity-based metrics such as `Shapley` improve perplexity, but severely degrade performance on other tasks such as MMLU, highlighting tension between relevance of different blocks.
% When looking at a finer granularity, our results highlight that self-attention layers in language models are more amendable to pruning as compared to feed-forward layers, where performance is unaffected by pruning a large number of self-attention layers in contrast to feed-forward layers.
% Finally, we look at bridging the misalignment introduced by block pruning using basic performance recovery techniques.
% Our simplest baseline of just using an average update achieves either comparable performance or outperforms the more powerful baseline of low-rank adapters with different formulations for training.

This paper explores depth pruning of LLMs, highlighting performance differences with various influence techniques, including adaptive ones. Block-sensitivity metrics like Shapley improve perplexity but degrade performance on tasks like MMLU, showing block relevance tension. Our results indicate self-attention layers are more amenable to pruning than feed-forward layers, with performance unaffected by pruning many self-attention layers. We also address misalignment from block pruning using basic performance recovery techniques. Our simplest baseline, using an average update, matches or outperforms low-rank adapters with different training formulations.

\paragraph{Limitations.}
One major limitation is the generalization to other datasets as we train and evaluate our approach on a single dataset i.e., OpenWebText~\citep{openwebtext}.
Changing the dataset can have a significant impact on performance.
However, our results are aligned with prior work that focuses on a different dataset for statistics computation~\citep{men2024shortgpt,gromov2024unreasonable}, highlighting robustness against changes in the data distribution.
Furthermore, we restrict most of our experiments to the evaluation of MMLU accuracy and OpenWebText perplexity following prior work~\citep{men2024shortgpt,gromov2024unreasonable} due to computational constraints.
This provides an incomplete picture of the actual impact of pruning on model performance as partially shown in Fig.~\ref{fig:llama2_harness} and Fig.~\ref{fig:mistral_harness}.


==> sections/experiments.tex <==
\section{Experiments}


\begin{figure*}[t]
    \centering
    \subfloat{
        \includegraphics[width=\textwidth]{figures/block_pruning_loss_shapley_10_05_24/block_pruning_llama-2_pretrained.pdf}
    }

    \vspace{-3mm}
    \subfloat{
        \includegraphics[width=\textwidth]{figures/block_pruning_loss_shapley_10_05_24/block_pruning_mistral_pretrained.pdf}
    }
    \caption{\textbf{Comparison of different block influence metrics} (detailed in Section~\ref{subsec:block_inf_metrics}) used for block pruning and their impact on downstream performance on LLaMa-2 7b (top) and Mistral 7b (bottom) in terms of average loss on a small curated validation set from OpenWebText and accuracy on MMLU.}
    \label{fig:metrics_comparison}
    \vspace{-5mm}
\end{figure*}


\begin{figure*}[t]
    \centering
    \subfloat{
        \includegraphics[width=\textwidth]{figures/layer_influence_loss_shapley_10_05_24/layer_pruning_both_mistral.pdf}
    }

    \vspace{-3mm}
    \subfloat{
        \includegraphics[width=\textwidth]{figures/layer_influence_loss_shapley_10_05_24/layer_pruning_mhsa_mistral.pdf}
    }

    \vspace{-3mm}
    \subfloat{
        \includegraphics[width=\textwidth]{figures/layer_influence_loss_shapley_10_05_24/layer_pruning_mlp_mistral.pdf}
    }
    \caption{\textbf{Comparison of different layer influence metrics on Mistral 7b} (detailed in Section~\ref{subsec:block_inf_metrics}) and their impact on downstream performance in terms of average loss on a small curated validation set from OpenWebText and accuracy on MMLU. The first row highlights joint pruning, while the second and third row highlights pruning of just self-attention or feed-forward layer respectively.} %\PM{quite interesting result! It seems that MHSA only pruning with Shapley should be better than cosine for full blocks, right? Comparing Figure 1 and Figure 5 it seems that you already have improvements by pruning both layers independently. }}
    \vspace{-5mm}
    \label{fig:layer_influence_mistral}
\end{figure*}


\begin{figure*}[t]
    \centering
    \subfloat{
        \includegraphics[width=\textwidth]{figures/metrics_comparison_05_04_23/block_pruning_llama-2_pretrained_emulated_update_relative.pdf}
    }

    \vspace{-3mm}
    \subfloat{
        \includegraphics[width=\textwidth]{figures/metrics_comparison_05_04_23/block_pruning_mistral_pretrained_emulated_update_relative.pdf}
    }
    \caption{\textbf{Relative impact on performance with emulated update as a performance recovery method.} The plot with the original values is presented in Fig.~\ref{fig:emulated_update}.}
    \label{fig:emulated_update_relative}
    \vspace{-5mm}
\end{figure*}


\begin{figure*}[t]
    \centering
    \subfloat{
        \includegraphics[width=\textwidth]{figures/linear_adapters_24_04_24/block_pruning_mistral_linear_adapter_r_8_representation_relative.pdf}
    }

    \vspace{-3mm}
    \subfloat{
        \includegraphics[width=\textwidth]{figures/linear_adapters_24_04_24/block_pruning_mistral_linear_adapter_r_8_sft_relative.pdf}
    }

    \vspace{-3mm}
    \subfloat{
        \includegraphics[width=\textwidth]{figures/linear_adapters_24_04_24/block_pruning_mistral_linear_adapter_r_8_logit_distillation_relative.pdf}
    }
    \caption{\textbf{Evaluating the relative impact of linear adapters for Mistral 7b with a rank of 8} trained using three different metrics including (a) MSE loss defined on the representation, (b) supervised fine-tuning (SFT), and (c) logit distillation where logits are distilled from the full model. The plot with the original values is presented in Fig.~\ref{fig:linear_adapters_rank_8_mistral}.}
    \label{fig:linear_adapters_rank_8_mistral_relative}
    \vspace{-5mm}
\end{figure*}


We use a subset of $150k$ sequences (context window of 2048 tokens) with cross-document concatenation from OpenWebText~\citep{openwebtext} as our full calibration set.
We use either the full or a subset of these documents to compute statistics or training.
We use another set of $\sim 15k$ sequences as a validation set to report loss/perplexity in the paper.
For block pruning, we rank all the blocks in the model with increasing order of influence and prune from the remaining blocks the ones with the least influence~\citep{men2024shortgpt,gromov2024unreasonable}.
The performance of the model on downstream tasks is evaluated at each successive pruning step which reduces the depth of the network by one block.
Note that it might be beneficial to recompute the block influence scores, particularly for adaptive techniques (similar to iterative pruning~\cite{tan2020dropnet}). However, we only evaluate one-shot influences in this paper by computing them once before pruning.
Furthermore, we evaluate the weighted accuracy of the model on Massive Multitask Language Understanding~\citep{hendrycks2020mmlu} which is a knowledge-intensive task.
For MMLU accuracy computation, we follow the original recipe from~\citet{hendrycks2020mmlu} including the prompt and directly compute the relative probabilities of generating the different options rather than using a generative evaluation.
We report 5-shot accuracy as commonly reported in the literature~\citep{touvron2023llama2,jiang2023mistral,men2024shortgpt,gromov2024unreasonable}.
We further evaluate performance on a range of different tasks mainly reported on OpenLLM leaderboard~\citep{open-llm-leaderboard} using eval-harness~\citep{eval-harness}.

We use LLaMa-2 7b~\citep{touvron2023llama2} and Mistral 7b~\citep{jiang2023mistral} for our evaluations.
We focus on 7b models primarily due to them being a sweet spot between compute cost and model quality.
Larger models are more amenable to block pruning, as already established in prior work~\citep{men2024shortgpt,gromov2024unreasonable}.
Therefore, we expect our findings to be equally applicable to larger models (if not more).
Due to limited space, we primarily focus on Mistral and include LLaMa-2 results where possible. The remaining results for LLaMa-2 are presented in Appendix~\ref{appendix:llama_remaining_results}.
% \PM{Picking one model is the right decision. Mistral seems to be a bit more robust - should be a better choice. We can show LlaMa additionally for some experiments in case there are different observations for both models.}


\subsection{Block influence metrics}

We compare different block influence metrics in Fig.~\ref{fig:metrics_comparison} for both LLaMa-2 7b~\citep{touvron2023llama2} and Mistral 7b~\citep{jiang2023mistral}, where we apply min-max normalization on the block influences for visualization (pruning is based on relative block ranking rather than the actual magnitude).
As cosine distance-based block influence matches the proposed approach in~\citep{men2024shortgpt,gromov2024unreasonable}, our results also closely match theirs in terms of robustness against block pruning.
Furthermore, the blocks that are assigned the least importance are located towards the end of the network i.e., the second half.
Relative $L_{p}$ norm metrics also closely follow this trend, and hence, achieve robustness comparable to that of cosine distance.

A significant deviation however is shown by the Shapley-value-based estimation, which is an adaptive metric that takes into account the task, providing significant gains in terms of reduction of the average loss (and hence perplexity) as it is specifically computed to reduce the model's language modeling loss.
However, this results in a drastic reduction in accuracy when evaluating MMLU.
Block influence plots show that in contrast to all other metrics that primarily focus on the second half of the network for removal, Shapley instead focuses on removing blocks from the first half of the network.
This, despite improving performance in terms of perplexity, results in an immediate loss of the model's ability to do well on knowledge-intensive tasks.
Therefore, these results highlight that task-specific (Shapley-based) block dropping might retain higher performance at the same number of dropped blocks as compared to task-agnostic techniques but at the expense of sacrificing more performance on tasks not directly considered.

We also visualize the results for Mistral-7b on other tasks from OpenLLM leaderboard~\citep{open-llm-leaderboard} using lm-eval-harness~\citep{eval-harness} in Fig.~\ref{fig:mistral_harness}.
These results highlight that despite just a relatively minor impact on performance for MMLU, some metrics are significantly more impeded (such as GSM-8k).
The proxy used in this case i.e., `cosine`, matches closely the right influence values to optimize MMLU, which is not aligned with the importance ideal for other datasets.
On the other hand, adaptive metrics can be optimized individually for each task at hand.

We further visualize the evolution of these metrics during model training using intermediate checkpoints provided for Pythia 2.8B model~\citep{biderman2023pythia}.
These results are presented in Appendix~\ref{appendix:pythia_cosine_over_time}.


\subsection{Disentangling the impact of individual layers}

As each block in a transformer is composed of self-attention as well as a feed-forward network, one can apply the same influence techniques to understand the impact of performance when pruning individual layers rather than complete blocks.
The results for Mistral are highlighted and Fig.~\ref{fig:layer_influence_mistral} (see Fig.~\ref{fig:layer_influence_llama2} for LLaMa-2 results).
We explore joint layer ranking (using scores for both self-attention and feed-forward networks -- first row) as well as individual ranking for each type (second and third row) to understand their impact on performance.
Note that since the influence values are normalized separately for the second and third row, this loses important information regarding relative magnitude which is preserved in the first row due to joint normalization.

Focusing on the first row, performance is preserved in the first few layers.
The model performance is maintained up to about 15 layers as compared to block pruning where we see a small negative slope already at the start.
When looking closely at the performance when individually pruning either self-attention (second row), or feed-forward network (third row), we see that models exhibit higher resilience against the dropping of self-attention layers in contrast to feed-forward layers.
In contrast to all other experiments, loss shapley in this case achieves competitive influence as compared to other approaches, highlighting that it might be easier to estimate in contrast to feed-forward layers.
Furthermore, Mistral exhibits a higher propensity for self-attention layer removal compared to LLaMa-2.
% Note that it is also possible to reuse attention outputs from previous layers to reduce the impact of dropping self-attention layers, as evaluated before in the context of computer-vision~\citep{venkataramanan2023skipattention}.
% We leave this as an interesting avenue to explore in the future.

% Although most of the parameters of a transformer are present in the feed-forward layers, pruning the self-attention layer is equally useful as self-attention has a quadratic dependency on the sequence length as well as requires complex management of key-value caches at inference time that introduces a significant latency overhead~\citep{xiao2023streaminglm,nawrot2024dynamic}.
% Significant efforts have been made in the recent past to accelerate self-attention layers in a transformer that directly translates to a reduction in the wall-clock time for both training and inference~\citep{dao2022flashattention,dao2023flashattentionv2}.
% Therefore, these results highlight a direct avenue for high gains in model inference speed, without sacrificing model quality, that goes beyond considering individual blocks.
% We consider the development of sophisticated techniques that combine both block and layer pruning as it might be possible to only prune a single layer for some of the blocks as an exciting direction for future research.
Although most transformer parameters are in the feed-forward layers, pruning the self-attention layer is equally useful due to its quadratic dependency on sequence length and the complex management of key-value caches, which introduces significant latency~\citep{xiao2023streaminglm,nawrot2024dynamic}. Recent efforts to accelerate self-attention layers have reduced wall-clock time for training and inference~\citep{dao2022flashattention,dao2023flashattentionv2}. These results suggest high gains in inference speed without sacrificing model quality. Developing techniques that combine block and layer pruning, potentially pruning only a single layer in some blocks, is an exciting direction for future research.

We also visualize the norm of the updates applied by the self-attention and feed-forward layers of the network in Fig.~\ref{fig:layer_update_norm} in the appendix. Consistent with the pruning results, we see a more significant update norm for the feed-forward layer as compared to the self-attention layers, highlighting the propensity for the model to tolerate higher pruning ratios for the self-attention layers.


\subsection{Performance recovery techniques}

% \textcolor{red}{TODO: Consider a new performance recovery technique based on block reapplication i.e., reapply a retained block in place of the dropped block. This requires a notion of block similarity. One rudimentary way to realize this would be to compute the similarity of blocks based on the distance between output representations given random inputs.}

We evaluate two distinct performance recovery techniques as highlighted in Section~\ref{subsec:performance_recovery_techniques}.
The first is a simple emulated update, while the second is based on training a low-rank linear adapter.
Note that we present relative differences in performance in comparison to the cosine block influence as highlighted in Figure~\ref{fig:metrics_comparison}. Positive values here indicate an increase as compared to the cosine block influence-based pruning, while negative values represent a decrease.
The original results without relative change are presented in Appendix~\ref{appendix:remaining_results}.


\subsubsection{Emulated update}
\label{results:emulated_update}

% The results for emulated update are visualized in Fig.~\ref{fig:emulated_update_relative} (also presented in Fig.~\ref{fig:main} for a direct comparison).
% We visualize both the computed mean as well as the standard deviation for reference in Appendix~\ref{appendix_subsec:emulated_update_stats}.
% We see a clear improvement for both LLaMa-2 and Mistral at around 7 blocks in terms of average loss (lower) as well as MMLU accuracy (higher).
% These results highlight that there are only minor differences introduced by later blocks that can even be recovered using simple techniques such as the one employed here. However, using this mitigation technique is unable to change the tipping point in performance.
% In terms of metrics, `shapley` still assigns relatively low influence to the first half of the blocks, and hence suffers in terms of performance on MMLU.

The results for emulated update are shown in Fig.\ref{fig:emulated_update_relative} (and Fig.\ref{fig:main} for direct comparison). Both the computed mean and standard deviation are referenced in Appendix~\ref{appendix_subsec:emulated_update_stats}. We observe a clear improvement for LLaMa-2 and Mistral at around 7 blocks in terms of average loss (lower) and MMLU accuracy (higher). These results indicate minor differences introduced by later blocks can be recovered using simple techniques. However, this mitigation technique doesn't change the tipping point in performance. The shapley metric still assigns low influence to the first half of the blocks, resulting in lower MMLU performance.

\subsubsection{Low-rank linear adapters}

We trained all our adapters for 800 steps with an effective batch size of 8.
The loss curves highlighted in Appendix~\ref{appendix:linear_adapter_loss_curves} signify that training the model for longer should have a negligible impact on model performance.
Furthermore, our influence computation in this case is based on a smaller subset of the full calibration set for computational convenience.

We present the results for Mistral with an adapter rank of 8 in Fig.~\ref{fig:linear_adapters_rank_8_mistral_relative} (see Fig.~\ref{fig:linear_adapters_rank_8_llama2_relative} for results on LLaMa-2).
The results for ranks 32 and 256 closely follow the same trend, and are presented in Appendix~\ref{appendix:low_rank_remaining_relative_results}.
Since we again present the results on a relative scale, the original results for reference are presented in Appendix~\ref{appendix:low_rank_original_results}.

% As we are training a linear adapter on top of the model, this allows us to define another block influence metric based on the `block adapter loss` as highlighted in Section~\ref{subsec:linear_adapters}.
% This provides us with two adaptive influence estimation techniques i.e., `shapley` based influence and `block adapter loss` based influence.

% The figure highlights an intriguing behavior for the `block adapter loss` influence estimate where training the model using the loss on the representation immediately takes a hit on the model performance after pruning even a single block from the network.
% Looking at the influence values, we see that the adapter loss is mostly low and slowly increases over time due to the increase in the norm of the hidden representation.
% This immediately highlights the weakness of training using representation loss i.e., it overly focuses on later blocks that are not essential for model performance as highlighted by our prior results due to the increasing output norm.
% On the other hand, using either SFT or logit distillation provides a block influence profile that closely matches the other metrics.


The figure reveals an interesting behavior for the block adapter loss influence estimate, where model performance drops significantly after pruning even a single block. The adapter loss is generally low but increases over time due to the growing norm of the hidden representation. This underscores the weakness of training with representation loss, which overemphasizes later blocks that aren't essential for performance. Conversely, using either SFT or logit distillation provides a block influence profile that closely aligns with other metrics.

Furthermore, in contrast to our prior experiments, we see a positive impact of using the `shapley` based influence which considers the quality of a particular adapter to replace the original block by computing the change in the final logits.
The influence profile also closely matches all other metrics in this case.
As one would expect, we see the most dominant performance when using `block adapter loss` as the influence metric, closely followed by `shapley` i.e., adaptive metrics that take into account the contribution of the performance recovery technique.

One surprising thing to note is that the performance with a linear adapter is either comparable (LLaMa-2 7b) or worse (Mistral 7b) than the performance improvement observed by the simple emulated block update (Section~\ref{results:emulated_update}).
This can be partially attributed to the overfitting of the adapter on the training corpus, which is not reflective of the true pertaining distribution.
\citep{gromov2024unreasonable} observed a similar performance degradation when trying to do parameter-efficient fine-tuning after dropping blocks from Mistral as compared to LLaMa-2.


==> sections/intro.tex <==
\section{Introduction}

\begin{wrapfigure}{r}{0.5\textwidth}
\centering
\vspace{-5mm}
\includegraphics[width=0.48\textwidth]{figures/fig1/fig1_mistral.pdf}
\caption{\textbf{Our self-attention pruning, adaptive metrics, as well as emulated updates in comparison to cosine block pruning} visualized w.r.t. compression ratios on Mistral 7b.}
\label{fig:main}
\vspace{-5mm}
\end{wrapfigure}
The utility of training language models with an increasing number of parameters is currently undisputed~\citep{kaplan2020scalinglaws,brown2020gpt3,touvron2023llama2,jiang2023mistral}.
This has led to tremendous gains in performance, including the emergence of in-context learning~\citep{brown2020gpt3}.
However, aside from training, which is a one-time cost, deploying these models in production presents unique challenges, particularly high inference costs.
Therefore, efficiency research for language models has gained significant popularity in the recent past~\citep{frantar2022gptq,ashkboos2024slicegpt,van2023llmsurgeon,men2024shortgpt}.

A primary area of investigation for efficient inference is quantization, with most models now being deployed even in 4-bit quantization for efficient inference even on consumer hardware~\citep{frantar2022gptq,mlx2023}.
Furthermore, several works identified a strong propensity for language models to undergo unstructured/structured pruning without hampering performance~\citep{ashkboos2024slicegpt,van2023llmsurgeon}.
It is important to note that (unsurprisingly), a large portion of these works focus on extremely large and undertrained models\footnote{We call models under-trained following Chinchilla scaling laws~\citep{hoffmann2022chinchila} -- recent trend goes even beyond this.}.
An extreme form of structured pruning is full block pruning from a pretrained model. \citet{men2024shortgpt,gromov2024unreasonable} recently showed that it is possible to completely drop blocks from a range of pretrained language models based on cheap proxies for block importance/influence.

This paper explores this direction further by analyzing the impact of different metrics on block identification, specifically focusing on adaptive metrics such as the one based on Shapley value~\citep{shapley1953value} in addition to static ones such as cosine block influence mainly used in prior work~\citep{men2024shortgpt,gromov2024unreasonable}.
We further look at the impact of individual self-attention and the feed-forward layers, which together form a block as analyzed by prior work.
Finally, we evaluate the effectiveness of simple strategies for performance recovery, including a simple baseline of an additive bias (called `emulated update`) which is based on the empirical mean of the update applied by the block, as well as learning-based techniques such as the training of a low-rank adapter, following prior literature on layer-stitching~\citep{bansal2021layerstitching}.

We visualize our main findings in Fig.~\ref{fig:main} where `block cosine` represents the method employed in prior work~\citep{men2024shortgpt,gromov2024unreasonable}.
Note that the x-axis here represents the compression ratio computed based on the total number of layers. However, it does not represent an equal number of parameters being pruned as a block comprises both a self-attention as well as a feed-forward network.
The figure highlights that the model can tolerate a higher fraction of pruning for self-attention layers in comparison to feed-forward layers (or blocks).
Pruning self-attention layers can provide a significant boost in model efficiency due to the costly maintenance of KV-cache at inference time.
We further include an upper-bound on MMLU performance by iteratively computing Shapley directly on the MMLU test set to get a glimpse of the best possible performance when we only care about this task.
% Due to this inference cost, KV-cache reduction has been a significant topic of attention in the recent past~\citep{xiao2023streaminglm,nawrot2024dynamic}.
Our main findings can be summarized as:

\findingbox{
We highlight the impact of different block influence metrics on downstream model performance.
Our analysis reveals a trade-off in performance between tasks when evaluating adaptive metrics such as the one based on Shapley values~\citep{shapley1953value} (Fig.~\ref{fig:metrics_comparison}). Furthermore, we find that performance on some tasks degrades significantly, such as GSM-8k~\citep{cobbe2021gsm8k} even when pruning a single block from the model (Fig.~\ref{fig:llama2_harness} and Fig.~\ref{fig:mistral_harness}).}
\vspace{1mm}
\findingbox{We further dissect a block into attention and feed-forward layers to separately evaluate their influence, and highlight a higher propensity to prune attention layers in contrast to feed-forward layers (Fig.~\ref{fig:main} and Fig.~\ref{fig:layer_influence_mistral}) on MMLU task.}
\vspace{1mm}
\findingbox{We evaluate two simple performance recovery techniques. One is based on a simple empirical mean of the block update (Fig.~\ref{fig:main} and Fig.~\ref{fig:emulated_update_relative}), while the second one trains a low-rank linear adapter in place of the missing block (Fig.~\ref{fig:linear_adapters_rank_8_mistral_relative}). Surprisingly, our results show that applying a simple average block update is either competitive or superior in performance as compared to the learning-based approach potentially due to overfitting and catastrophic forgetting. In particular, we observe performance improvements by attaching a low-rank linear adapter for LLaMa-2 (Fig.~\ref{fig:linear_adapters_rank_8_llama2_relative}), but performance instead degrades for Mistral 7b (Fig.~\ref{fig:linear_adapters_rank_8_mistral_relative}) which is aligned with the results on model healing from~\citep{gromov2024unreasonable}.}


==> sections/methods.tex <==
\section{Methods}

We consider a regular transformer architecture with self-attention, feed-forward layers, and input layer-norms~\citep{vaswani2017transformer}. Let $\mathbf{H}^{l}$ represent the output from the $l^{th}$ block. Below, we describe the influence metrics and performance recovery techniques used in our experiments.


\subsection{Block influence metrics}
\label{subsec:block_inf_metrics}

\paragraph{Cosine block influence}, a prominent recent technique~\citep{men2024shortgpt,gromov2024unreasonable}, computes the cosine distance between a block's input and output representations. This involves averaging over examples and individual tokens indexed by $t$.
\begin{equation}
    I^{l}_{cosine} = 1 - \mathbb{E}_{\mathbf{X}, t} \frac{(\mathbf{H}^{l-1}_{t})^{T} \mathbf{H}^{l}_{t}}{\norm{\mathbf{H}^{l-1}_{t}} \norm{\mathbf{H}^{l}_{t}}}
\end{equation}

\paragraph{Relative $L_{p}$ update norm} is similar to cosine distance in spirit but computes the relative change in the norm induced by the block output.
\begin{equation}
    I^{l}_{p} = \mathbb{E}_{\mathbf{X}, t} \frac{\norm{\mathbf{H}^{l}_{t} - \mathbf{H}^{l-1}_{t}}_{p}}{\norm{\mathbf{H}^{l-1}_{t}}_{p}}
\end{equation}
We evaluate $p=1$ and $p=2$ in our case, naming them as relative $L_{1}$ and relative $L_{2}$ respectively.
Note that $p=2$ is similar to the metric from~\citep{samragh2023weightcloning,men2024shortgpt}, and is more susceptible to outliers compared to $L_{1}$.
We compute the relative update norm instead of directly using the update norm as the norm of update gradually increases throughout the forward propagation~\citep{liu2023dejavu} (see Fig.~\ref{fig:block_update_norm} in the appendix).

\paragraph{Shapley} leverages the game-theoretic Shapley value~\citep{shapley1953value} to determine each block's marginal contribution. We target Shapley values for distances to full model logits, language modeling loss with leave-one-out, and task-specific loss functions. Influential blocks yield large negative values, so we use the negative Shapley value as our block influence. 
In particular, for loss-based Shapley-value of a block, we compute the difference between the loss when a particular block is present and absent i.e.:
\begin{equation}
    % \textsc{SHAP}^{l} = \mathbb{E}_{\mathbf{X}, t, s \in S} \; \mathcal{L}(O^{s}) - \mathbb{E}_{\mathbf{X}, t, s \in S \setminus l} \; \mathcal{L}(O^{s})
    \textsc{SHAP}^{l} = \mathbb{E}_{\mathbf{X}, t, s \subseteq S \setminus \{l\}} \left[\mathcal{L}(O^{s \cup \{l\}}) - \mathcal{L}(O^{s})\right]
\end{equation}
\noindent where $S$ represents the full set of blocks, $s$ represents a subset of the blocks, and $O^{s}$ represents the output of the model using a subset of the blocks $s$.
As Shapley-value takes into account an objective, this makes them more adaptive to the task.
% Unlike other metrics, Shapley is dynamic and task-specific, whereas previous metrics are task-agnostic.
% Shapley values are more adaptive to different tasks because their calculation is dependent on a task-specific loss function.

\subsection{Performance recovery techniques}
\label{subsec:performance_recovery_techniques}

Dropping blocks from a pretrained model poses a risk of changing the norm of the activations for the model, and hence driving the activations to be out-of-distribution w.r.t. the subsequent blocks.
Therefore, we consider two simplistic techniques that attempt to maintain the norm of the activations.

\subsubsection{Emulated update}

Emulated update is a particularly simple strategy that computes the average update applied by each block on a small calibration set, and applies that average additive update at inference time when a particular block is dropped.
This can be viewed as having a `bias` term instead of the full block.
\begin{equation}
    \Delta \mathbf{H}^{l}_{avg} = \mathbb{E}_{\mathbf{X}, t} \;\; \big[ \mathbf{H}^{l}_{t} - \mathbf{H}^{l-1}_{t} \big]
\end{equation}
\begin{equation}
    \mathbf{H}^{l} = \mathbf{H}^{l-1}_{t} + \Delta \mathbf{H}^{l}_{avg}
\end{equation}
\noindent 


\subsubsection{Low-rank linear adapters}
\label{subsec:linear_adapters}

Block influence metrics, such as cosine~\citep{men2024shortgpt,gromov2024unreasonable} consider any blocks that apply a simple rotation of the representation space to be significant.
However, such a simple misalignment between layers can be simply recovered by training a small linear adapter and was previously explored for stitching layers of different models together~\citep{bansal2021layerstitching}.
Furthermore, low-rank adapters are now commonly employed for parameter-efficient fine-tuning of language models~\citep{hu2021lora}.

Combining these ideas, we evaluate the efficacy of training low-rank linear adapters as a performance recovery measure. More precisely, we introduce two new matrices per block to be learned (aside from the per-channel weightings learned as part of the normalization layer):
\begin{equation}
    \mathbf{H}^{l} = \mathbf{H}^{l-1}_{t} + \mathbf{W}_{b}^{T} \; ( \mathbf{W}_{a}^{T} \; \textsc{LN} (\mathbf{H}^{l-1}) )
\end{equation}
\noindent where $\mathbf{W}_{a} \in \mathbb{R}^{D \times r}$, $\mathbf{W}_{b} \in \mathbb{R}^{r \times D}$ with $r$ being the rank of the adapter, while $D$ being the embedding dimension of the transformer.
This is similar in spirit to the healing process based on LoRA adapters by~\citet{gromov2024unreasonable}.
However, we apply it in place of the missing blocks following the perspective of layer stitching, while \citet{gromov2024unreasonable} applied these low-rank adapters on the retained blocks.

We consider three different ways of training these linear adapters: (i) minimize MSE between the output of the block and the low-rank adapter, (ii) use supervised fine-tuning (SFT) on the final output, and (iii) use logit-distillation on the final model output.
We use a small calibration set to train this low-rank adapter independently one block at a time.

\paragraph{Block adapter loss.}
Training low-rank adapters offers a block influence metric based on their average training loss. This quantifies the quality of the adapter and the potential to replace the original block with it. We evaluate using block adapter loss as the model influence metric when attaching adapters to the model.


==> sections/methods_initial.tex <==
\section{Methods}

We formalize a $L$ blocks transformer as:

\begin{equation*}
    \mathbf{H}^{0} = \mathbf{W}_{E}^{T} \mathbf{X}
\end{equation*}
\begin{equation*}
    \mathbf{H}^{l}_{prime} = \mathbf{H}^{l} + \textsc{MHSA}( \textsc{LN} (\mathbf{H}^{l}) )
\end{equation*}
\begin{equation*}
    \mathbf{H}^{l+1} = \mathbf{H}^{l}_{prime} + \textsc{FFN}( \textsc{LN} (\mathbf{H}^{l}_{prime}) )
\end{equation*}
\begin{equation*}
    \mathbf{O}^{L} = \mathbf{W}_{U}^{T} \mathbf{H}^{L}
\end{equation*}

\noindent where $\textsc{MHSA}$ represents the self-attention layer, $\textsc{LN}$ represents the layer-norm\footnote{Note that LLaMa-2~\citep{touvron2023llama2} and Mistral 7b~\citep{jiang2023mistral} uses RMSNorm\xd{[cite]} instead of LayerNorm\xd{[cite]} in their models.
% However, this distinction is irrelevant for our purposes.
}, and $\textsc{FFN}$ represents the MLP, $\mathbf{W}_{E}$ represents the embedding matrix while $\mathbf{W}_{U}$ represents the unembedding matrix, $\mathbf{X}$ represents the input sequence, $\mathbf{O}^{L}$ represents the output sequence (one for each input token) when using all $L$ blocks of the model, and $\mathbf{H}$ represents the hidden representation of the model.

% Due to the residual nature of these block outputs where each subsequent block makes a small update to the representation from the previous block, dropping blocks from the model should have minimal impact on model performance.
% \xd{no need to mention this here.}


\subsection{Block influence metrics}
\label{subsec:block_inf_metrics}

We consider four different metrics.

\paragraph{Cosine block influence} is one of the most prominent techniques in the recent past~\citep{men2024shortgpt,gromov2024unreasonable} that computes the cosine distance between the input and the output representation from a block.

\begin{equation}
    I^{l}_{cosine} = 1 - \mathbb{E}_{\mathbf{X}, t} \frac{(\mathbf{H}^{l-1}_{t})^{T} \mathbf{H}^{l}_{t}}{\norm{\mathbf{H}^{l-1}_{t}} \norm{\mathbf{H}^{l}_{t}}}
\end{equation}

\noindent which computes an expectation over both different sequences as well as different tokens in a sequence indexed by $t$.

\paragraph{Relative $L_{p}$ update norm} is similar to cosine distance in spirit but computes the relative change in the norm induced by the block output.

\begin{equation}
    I^{l}_{p} = \mathbb{E}_{\mathbf{X}, t} \frac{\norm{\mathbf{H}^{l}_{t} - \mathbf{H}^{l-1}_{t}}_{p}}{\norm{\mathbf{H}^{l-1}_{t}}_{p}}
\end{equation}

We evaluate $p=1$ and $p=2$ in our case, naming them as relative $L_{1}$ and relative $L_{2}$ respectively.
\xd{use few sentences to explain l1 and l2 differences. l2 is more senstive to outlier updates?} 
Note that $p=2$ is similar to the metric from~\citep{samragh2023weightcloning,men2024shortgpt}.
We compute the relative update norm as compared to the direct update norm as the norm of update gradually increases throughout the forward propagation~\citep{liu2023dejavu} (see Fig.~\ref{fig:block_update_norm} in the appendix that visualizes the L2 norm of block updates for both LLaMa-2 and Mistral).

\paragraph{Shapley} leverages the game-theoretic notion of Shapley value~\citep{shapley1953value} to decide the marginal contribution of each of the blocks in the network.
In order to operationalize this, we propagate the input once through the full model and compute the final logits.
We then leave out one block at a time and compute the L2 distance to the full model logits. Finally, we compute the average of the distance in all cases where a block was present and subtract from it the distance in all cases where the block was absent. More precisely:

\begin{equation}
    \textsc{shap}^{l} = \mathbb{E}_{\mathbf{X}, t, S \setminus l} \norm{\mathbf{O}_{t} - \mathbf{O}^{S \cup l}_{t}} - \mathbb{E}_{\mathbf{X}, t, S \setminus l} \norm{\mathbf{O}_{t} - \mathbf{O}^{S}_{t}}
\end{equation}

\noindent where $\mathbf{O}_{t}$ represents the complete model output at position $t$, while $\mathbf{O}_{t}^{S}$ represents the model output when using a subset $S$ of the total blocks in the model. We use leave-one-out estimation for our evaluation i.e., $|S| = L-1$.
This definition also resembles per-example influence estimation that attempts to infer the relative importance of different data points present in a dataset~\citep{feldman2020memorization}.\xd{Why we want to mention this?}
Note that since this metric quantifies the contribution of a block in reducing the distance to the full model logits, most influential blocks should yield a large negative value.
Hence, we use the negative of this estimate as our block influence measure i.e., $I^{l}_{cosine} = \textsc{shap}^{l}$.

\textcolor{red}{TODO: Update to accommodate the description for loss shapley.}


\subsection{Performance recovery techniques}
\label{subsec:performance_recovery_techniques}

Dropping blocks from a pretrained model poses a risk of changing the norm of the activations for the model, and hence driving the activations to be out-of-distribution w.r.t. the subsequent blocks.
Therefore, we consider two simplistic techniques that attempt to maintain the norm of the activations.

\subsubsection{Emulated update}

Emulated update is a particularly simple strategy that simply computes the average update applied by each block on a small calibration set, and applies that average additive update at inference time when a particular block is dropped. More precisely, we first compute the average update for a particular block $l$:

\begin{equation}
    \mathbf{H}^{l}_{avg} = \mathbb{E}_{\mathbf{X}, t} \;\; \big[ \mathbf{H}^{l}_{t} - \mathbf{H}^{l-1}_{t} \big]
\end{equation}
\xd{You use $\mathbf{H}$ to represent output. So here it should be $\Delta \mathbf{H}^l_{avg}$.}

\noindent The computed average update is then applied to the representation at inference time instead of the block itself once it is dropped:

\begin{equation}
    \mathbf{H}^{l} = \mathbf{H}^{l-1}_{t} + \mathbf{H}^{l}_{avg}
\end{equation}

This can be viewed as just having a `bias` term instead of the full block.
Note that the emulated update can potentially fail to maintain the norm in case of high variance i.e., conflicting updates on a particular channel resulting in a cancellation of the update itself.
\xd{cannot follow the last sentence.}

\subsubsection{Low-rank linear adapters}
\label{subsec:linear_adapters}

Block influence metrics, such as cosine~\citep{men2024shortgpt,gromov2024unreasonable} consider any blocks that apply a simple rotation of the representation space to be significant.
However, such a simple misalignment between layers can be simply recovered by training a small linear adapter and was previously explored for stitching layers of different models together~\citep{bansal2021layerstitching}.

Furthermore, low-rank adapters are now commonly employed for parameter-efficient fine-tuning of language models~\citep{hu2021lora}.
Therefore, combining these ideas, we evaluate the efficacy of training low-rank linear adapters as a performance recovery measure. More precisely, we introduce two new matrices per block to be learned:

\begin{equation}
    \mathbf{H}^{l} = \mathbf{H}^{l-1}_{t} + \mathbf{W}_{b}^{T} \; ( \mathbf{W}_{a}^{T} \; \textsc{LN} (\mathbf{H}^{l-1}) )
\end{equation}

\noindent where $\mathbf{W}_{a} \in \mathbb{R}^{D \times r}$, $\mathbf{W}_{b} \in \mathbb{R}^{r \times D}$ with $r$ being the rank of the adapter, while $D$ being the embedding dimension of the transformer.
This formulation is similar in spirit to the healing process based on LoRA adapters proposed by~\citet{gromov2024unreasonable}.
However, we apply it in place of the missing blocks following the perspective of layer stitching, while \citet{gromov2024unreasonable} applied these low-rank adapters on the retained blocks.

One way to train these low-rank adapters is to apply the loss to the output representation of the block i.e.,

\begin{equation}
    \mathcal{L} = \mathbb{E}_{\mathbf{X}, t} \norm{\mathbf{W}_{b}^{T} \; ( \mathbf{W}_{a}^{T} \; \textsc{LN} (\mathbf{H}^{l-1}) ) - \mathbf{H}^{l}_{t}}
\end{equation}

\noindent where $\mathbf{H}^{l}_{t}$ represents the representation of the model obtained by applying the original block $l$ to the previous representation.
This loss attempts to minimize the difference in the representation between the actual block output and the low-rank adapter output.

The second way to train is to just use supervised fine-tuning with the block replaced with the low-rank adapter as done in~\citep{gromov2024unreasonable}.

Finally, the third way to train is to use logit-distillation where we compute the logits using the full model, and then minimize the difference between logits when using an adapter in the middle instead of the original block $i$~\citep{hinton2015distilling,joseph2020logit}. Note that this is computationally the most expensive, and requires two forward passes through the full model\footnote{It is possible to cache logits from the original model. However, we ignore that in this work as we train for a fixed number of steps on distinct examples, diminishing the utility of pre-caching.}

Again, we use a small calibration set to train this low-rank adapter independently one block at a time.

\paragraph{Block adapter loss.}
Training these low-rank adapters provides another block influence metric which is simply the average loss of the adapter during training.
This quantifies the quality of our adapter and hence dictates the ability for the original block to be replaced with this low-rank adapter. Therefore, we also evaluate the utility of using our block adapter loss as the model influence metric when attaching block adapters to the model.


==> sections/related_work.tex <==
\section{Related work}
\label{sec:related_work}

\citet{he2016resnets} popularized residual layers for training deep models, enabling residual networks to be seen as ensembles of smaller sub-networks~\citep{veit2016resnetsasensembles}. This led to layer dropping at inference time with minimal performance loss. \citet{veit2018convaig} extended this to dynamic input-conditioned layer-skipping.

\citet{vaswani2017transformer} introduced the famous transformer architecture that combined ideas of attention and residual networks to develop highly performant architectures for natural-language translation tasks.
Subsequent work analyzed and established the general utility of this architecture for a range of different tasks including state-of-the-art language models~\citep{touvron2023llama2,jiang2023mistral}, computer vision models~\citep{kirillov2023segmentanything}, as well as weather forecasting systems~\citep{bi2022pangu}.
Due to the high cost of serving these models, particularly LLMs, recent work attempted to understand and prune layers from a pretrained language model to accelerate model inference.
While there is a large body of work on pruning, we  focus on depth pruning and refer the readers to \citet{wan2023efficientllms} for a more comprehensive treatment of the literature.

\citet{samragh2023weightcloning} initialized a subnetwork from a larger pretrained network by identifying the most important blocks to retain using the relative norm of the block update. They argued that the best layers to remove are in the middle of the network for GPT-2 trained on Pile.
Sheared LLaMa~\citep{xia2023shearedllama} proposed an optimization-based view for pruning LLaMa-2 7b model~\citep{touvron2023llama2} including both depth and width pruning for pretrained models. They also utilized extensive fine-tuning of a low-rank adapter as a performance recovery technique.
Shortened LLaMa~\citep{kim2024shortenedllama} focused particularly on depth pruning, and showed that to be competitive against width-only pruning, or a sophisticated combination of both.
They constructed proxy metrics for block influence estimation primarily based on the weights of the network.
One of the considered metrics was based on the drop in perplexity, which resembles our loss-shapley on the language modeling task.

% Their criterion for block importance is based on $\frac{\norm{f(x)}}{\norm{f(x) + x}}$, which goes to 0 when the block is unimportant. We call this relative l2 metric which computes the relative change applied by the model on the input representation.
\citet{men2024shortgpt} extended this analysis to LLaMa-2~\citep{touvron2023llama2} by using cosine distance (between activations before and after a block) as a proxy of block importance.
\citet{gromov2024unreasonable} also showed similar results on both LLaMa-2~\citep{touvron2023llama2} and Mistral~\citep{jiang2023mistral}, while also proposing a healing method by optimizing low-rank adapters~\citep{hu2021lora} for the remaining blocks. This healing process is aimed at minimizing performance degradation with block pruning.
% FFN-skip ref: https://arxiv.org/pdf/2404.03865.pdf
\citet{jaiswal2024ffnskipllm} extended the cosine distance in a dynamic manner by computing the cosine similarity of the representations at inference time, and skip only the feed-forward layers in the less important regions of the network (particularly in the middle of the network).

In a similar spirit, \citet{raposo2024mixtureofdepths} trained a router to decide which blocks to skip i.e., reduce network depth (similar to the expert router in MoE~\citep{shazeer2017mixtureofexperts}). In contrast to other adaptive computing techniques, they leverage a static graph by fixing the number of tokens that can be processed through that block to 50\%, and select the top 50\% with the highest selection scores from the router. 
% As this approach requires computing information regarding the selection scores for all other tokens which is unavailable at inference time, they train a predictor to predict whether a token would be within top-k directly that can be used at inference time.

This paper attempts to take a deeper look at depth pruning of LLMs by looking at multiple metrics, datasets, block granularities (going to individual feed-forward and self-attention layers), and recovery techniques to establish the utility of each of these decisions on the resulting model.


==> sections/todo_list.tex <==
\section{TODO list}

List of TODOs:

\begin{itemize}
    \item Introduce a learnable approach for the block influence. We tested block sigmoid as well as Gumbel-Sigmoid/Softmax, but none of these approaches seem to work well for this purpose.
    \item Introduce the base where we just randomly search for networks on MMLU (subsampling the dataset might be detrimental in this case).
    \item Try to change the MMLU shapley computation to use the train set rather than the test set.
    \item Block reapplication? Can we do better is we allow reapplication of a block?
    \item MLP pruning is worse than pruning entire blocks. Two possible explanations are: (i) cosine as a proxy works well for full blocks, but fails for MLPs i.e., a better MLP influence metric should achieve performance comparable to that of full block pruning, (ii) removing MLPs while retaining attention produces OOD outputs for subsequent layers, immediately plummeting performance which necessitates removal of both self-attention and feed-forward layer simultaneously.
\end{itemize}

